Photoevaporation of Grain-Depleted Protoplanetary Disks around Intermediate-Mass Stars: Investigating Possibility of Gas-Rich Debris Disks as Protoplanetary Remnants

Debris disks are classically considered to be gas-less systems, but recent (sub)millimeter observations have detected tens of those with rich gas content. The origin of the gas component remains unclear; namely, it can be protoplanetary remnants and/or secondary products deriving from large bodies. In order to be protoplanetary in origin, the gas component of the parental protoplanetary disk is required to survive for $\gtrsim10{\,\rm Myr}$. However, previous models predict $\lesssim 10{\,\rm Myr}$ lifetimes because of efficient photoevaporation at the late stage of disk evolution. In the present study, we investigate photoevaporation of gas-rich, optically-thin disks around intermediate-mass stars at a late stage of the disk evolution. The evolved system is modeled as those where radiation force is sufficiently strong to continuously blow out small grains ($\lesssim 4 {\,\rm \mu m}$), which are an essential component for driving photoevaporation via photoelectric heating induced by stellar far-ultraviolet (FUV). We find that the grain depletion reduces photoelectric heating, so that FUV photoevaporation is not excited. Extreme-ultraviolet (EUV) photoevaporation is dominant and yields a mass-loss rate of $2$--$5\times10^{-10}(\Phi_{\rm EUV}/10^{41}{\,\rm s}^{-1})^{1/2}\,M_\odot\,{\rm yr}^{-1}$, where $\Phi_{\rm EUV}$ is the EUV emission rate. The estimated lifetimes of the gas component are $\sim 50 (M_{\rm disk}/10^{-2}\,M_\odot)(\Phi_{\rm EUV}/10^{41}\,{\rm s}^{-1})^{1/2}\,{\rm Myr}$ and depend on the ``initial'' disk mass at the point small grains have been depleted in the system. With an order estimation, we show that the gas component can survive for a much longer time around A-type stars than lower-mass stars. This trend is consistent with the higher frequency of gas-rich debris disks around A-type stars, implying the possibility of the gas component being protoplanetary remnants.

==> ingredients.tex <==
\if0
        \begin{table*}[htp]
                \caption{Model Parameters}
                \begin{center}
                \begin{tabular}{l    c |c | c}   
                &G-type PMS star& A-type MS star (Appendix?) & A-type star (49 Ceti; fiducial) \\ \hline \hline
                [{\it Stellar parameters}]                                                       \\
                Mass $(M_*)$     				&               $ 1.0  \Msun$ & $ 3.0  \Msun$ 
                &      $2.0\Msun$                            \\
                Radius $(R_*)$                          &               $ 2.61 \Rsun$ & $ 1.6 \Rsun$
                &         $1.88\Rsun$                                                            \\
                FUV luminosity $(\LFUV)$        &               $ 6\e{30}\unit{erg}{}\unit{s}{-1}$   & $ 1.5\e{34}\unit{erg}{}\unit{s}{-1}$
                & $3.01\e{33}$                                     \\
                EUV emission rate $(\LEUV)$     &               $  1\e{41}\unit{s}{-1}$ & $  4\e{41}\unit{s}{-1}$
                & $5.31\e{40}$                                                 \\      
                X-ray luminosity $(L_{\rm X})$	&		$1\e{30} \erg \sec^{-1}$ & $1\e{29} \erg \sec^{-1}$
                & $1\e{29} \erg \sec^{-1}$	\\	
                \hline
                [{\it Disk parameters}]                                                       \\
                Configuration				&	Full	&	Full	&	Truncated	\\
                Truncated radius $(R_{\rm min})$  	& --	& -- &   $25\au$\\
                Outer extent $(R_{\rm max})$	&		\multicolumn{3}{c}{$20 \, R_{\rm g}$}	\\	
				Disk mass $(M_{\rm disk})$  &  $   \Msun$ & $   \Msun$ & $0.001\Msun$\\
                \hline
                [{\it Gas/dust properties}]                                                     \\
                Gas species                                     & \multicolumn{3}{c}{H, \ce{H+}, \ce{H2}, \ce{H2+}, CO, O, \ce{C+}, \ce{e-} }     \\
                Carbon abundance $(\abn{C})$&                   \multicolumn{3}{c}{$ 0.927\e{-4} $}                                        \\
                Oxygen abundance $(\abn{O})$&                   \multicolumn{3}{c}{$ 3.568\e{-4} $}                                         \\      
                Dust-to-gas mass ratio $(\dgratio)$             &       \multicolumn{3}{c}{$ 0.01 $}       \\
                Maximum grain size ($a_{\rm max}$)		&		$1\mum$ & \multicolumn{2}{c}{$10\mum$} \\
                Minimum grain size ($a_{\rm min}$)		&		\multicolumn{3}{c}{$1\e{4}\mum	$}	\\
                \hline
                \end{tabular}
                \end{center}
                \label{tab:model}
        \end{table*}
\fi

\if0
        A hybrid scheme is adopted; 
        ray tracing is used to calculate the radiative transfer for 
        the direct component (stellar irradiation),
        while a flux-limited-diffusion (FLD) approximation is used 
        to solve the radiative transfer of the diffusion component
        coming from thermal (re-)emission by dust. 
        The radiation transport module of \cite{2010_Kuiper} 
        is used for the radiative transfer calculations.
        The temperature distribution of dust can be accurately modeled 
        even in an optically-thick region with the hybrid scheme \citep{2013_Kuiper}.
        Strictly speaking, the FLD approximation is not valid 
        in optically-thin disk wind regions ($\Av < 1$).
        However, the stellar irradiation component dominates the local radiation field there. 
%       the stellar irradiation directly illuminates the region;
%       hence, the stellar irradiation component dominates the local radiation field  
%       rather than the diffuse component.
        The base region ($\Av \sim 1$)
%       the direct field is attenuated to some extent, 
%       but the region is optically thin to the diffusion component.
        is optically thin to the diffusion component although it partially attenuates 
        the direct component. 
        The dust temperatures in such region are largely set by the direct irradiation as the wind region.
        We have explicitly checked that 
        including the diffusion component does not change 
        the derived dust temperatures. 
        The difference is only $\sim 2\%$ on average, and at most $6\%$.
        Therefore, it is concluded that our radiative transfer calculations 
        can model an accurate temperature distribution of dust grains.
%       we conclude that our calculations give
%       accurate dust temperatures in the wind regions.
        It is noteworthy that 
        the radiative transfer method has been applied 
        to studies in many different context,
        such as massive star formation and feedback effects
        \citep{2010_Kuiper2,2012_Kuiper,2013_Kuiper_ab,2015_Kuiper,2016_Kuiper},
        stellar evolution \citep{2013_KuiperYorke},
        the formation of primordial stars \citep{2016_Hosokawa},
        massive accretion disks \citep{2011_Kuiper,2017_Meyer, 2017_Meyer_aa},
        and planet formation \citep{2017_Marleau}.

        We use the opacity table provided by \cite{1984_DraineLee}
        for the radiative transfer calculations.

        
        The absorption of the direct EUV from the central star 
        is considered.          
        The radiative transfer equation for the absorption is
        \eq{
                \frac{1}{r^2} \partialdif{}{r} \braket{ r^2 F_\nu } 
                = - n_{\HImath} \sigma_\nu F_\nu  , \label{eq:rteuv}
        }
        where $\nu $ is an EUV photon frequency,  
        $F_\nu$ is the specific number flux of the direct EUV field,
        $\nspe{\HImath}$ is the atomic hydrogen density, 
        and $\sigma_\nu$ is the absorption cross section of \HI. 
        We adopt the approximated absorption cross-section  
        \eq{
                \sigma_\nu 
                = 6.3\e{-18} \braket{\frac{h\nu}{h\nu_1}}^{-3}\cm^2, 
                \label{eq:crosssectioneuv}
        }
        \citep[e.g.,][]{2006_OsterbrockFerland}.
        In \eqnref{eq:crosssectioneuv},
        $\nu_1$ is the Lyman limit frequency 
        ($h\nu_1 \simeq 13.6\eV; \lambda_1 \equiv c/\nu_1 \simeq 91.2  {\rm \, nm}$). 
        The solution of \eqnref{eq:rteuv} is analytically calculated as
        \eq{
                F_\nu (r,\theta,t)
                = \frac{\LEUV}{4\pi r^2} 
                \exp \left[{-\sigma_\nu N_{\HImath}}\right] , \label{eq:speflux}
        }
        where $N_{\HImath} = N_{\HImath}(r,\theta,t)$ is 
        the column density of atomic hydrogen
        measured from the stellar surface
        \eq{
                N_{\HImath}(r, \theta,t)  \equiv \int 
                dr' \, \nspe{\HImath}(r',\theta,t) .
        }
        \eqnref{eq:speflux}
        provides the photoionization rate 
        and the associated heating rate
        \gathering{
                         R_{\rm Ionize}                 
                        = \abn{\HImath} \int _{\nu_1}^{\infty} 
                        {\rm d}\nu \, \sigma _\nu F_\nu  , \label{eq:ioni} \\
                         \Gamma_{\rm EUV}       =  \frac{\nspe{\HImath}}{\rho} 
                 \int _{\nu_1}^{\infty} {
                        \rm d}\nu \, \sigma _\nu h(\nu-\nu_1)F_\nu  ,
        }
        respectively. 
        We assume a black body spectrum for the SED of the EUV.
        The effective temperature is set to $T_{\rm eff} = 10^4 \Kelvin$,
        which yields the total stellar EUV emission rate of 
        $\LEUV \simeq 1.5\e{41} (R_*/\Rsun)^2 \unit{s}{-1}$.
        The frequency-integration range is divided into 81 bins.
 \fi    

        \begin{table}[htp]
                \caption{Model Parameters}
                \begin{center}
                \begin{tabular}{l c c}   
                &A-type (fiducial) % (49 Ceti; fiducial) 
                &G-type   \\ \hline \hline
                [{\it Stellar parameters}]                                                       \\
                Mass $(M_*)$     				& $ 2  \Msun$ &      $1\Msun$                            \\
                Radius $(R_*)$                 	& $1.88\Rsun$ 	&	$ 2.61 \Rsun$ \\
                Bolometric luminosity  $(L_*)$  &   $19\Lsun$   &   $2.3 \Lsun$\\
                FUV luminosity $(\LFUV)$        & $3.01\e{33}\unit{erg}{}\unit{s}{-1}$  &$ 6\e{30}\unit{erg}{}\unit{s}{-1}$ \\
                EUV emission rate $(\LEUV)$     & $5.31\e{40}\sec^{-1}$  &$  1\e{41}\unit{s}{-1}$      \\      
                X-ray luminosity $(L_{\rm X})$	& $1\e{29} \erg \sec^{-1}$ & $1\e{30} \erg \sec^{-1}$ 	\\	
                \hline
                [{\it Disk parameters}]                                                       \\
                Configuration					&	\multicolumn{2}{c}{Truncated at $R_{\rm min} = 25\au$ or Full}	\\
%                Truncated radius $(R_{\rm min})$&	\multicolumn{2}{c}{$25\au$/--}	\\
                Outer extent $(R_{\rm max})$	&		\multicolumn{2}{c}{$20 \, R_{\rm g}$}	\\	
				Disk mass $(M_{\rm disk})$  	&    \multicolumn{2}{c}{$10^{-3}$--$10^{-2}\Msun$} \\
                \hline
                [{\it Gas/dust properties}]                                                     \\
                Gas species                                     & \multicolumn{2}{c}{H, \ce{H+}, \ce{H2}, \ce{H2+}, CO, O, \ce{C+}, \ce{e-} }     \\
                Carbon abundance $(\abn{C})$&                   \multicolumn{2}{c}{$ 0.927\e{-4} $}                                        \\
                Oxygen abundance $(\abn{O})$&                   \multicolumn{2}{c}{$ 3.568\e{-4} $}                                         \\      
                Dust-to-gas mass ratio              &       \multicolumn{2}{c}{$ 0.01 $}       \\
                Min. grain size ($a_{\rm max}$)		&	$10\mum$ & 	$1\mum$ \\
                Max. grain size ($a_{\rm min}$)		&		\multicolumn{2}{c}{$1\cm$--$100\km$}	\\
                \hline
                \end{tabular}
                \end{center}
                \label{tab:model}
        \end{table}


\if0
        {\small
\begin{longtable}[htp]{ll p{6cm} c }
%\begin{center}
\caption{The List of the Chemical Reactions Incorporated in Our Simulations% \\[3mm]
}\\ \hline
%\begin{tabular}{lllc}\hline
Label   & Reaction      
%& Rate Coefficient\, $^a$ & Reference\,$^b$\\ \hline \hline
& Rate Coefficient & Reference \\ \hline \hline
\endfirsthead
\multicolumn{4}{r}{\tref{tab:chem_reac} Continued}      
\\      \hline
Label   & Reaction      &
% Rate Coefficient\, $^a$ & Reference\,$^b$\\ \hline \hline
 Rate Coefficient & Reference \\ \hline \hline
\endhead
\hline
\multicolumn{4}{r}{Continued}
\\
\endfoot
\hline
%\multicolumn{4}{r}{End}
% \multicolumn can write words which use several columns. 
\multicolumn{4}{p{14cm}}{
{\bf Note:} Here $\TeV$ is the gas temperature in ${\rm eV}$, $T$ is the gas temperature in ${\rm K}$,
and $T_{\rm dust}$ is the dust temperature in ${\rm K}$;
{\bf References:} (1) \cite{2000_Omukai}, (2) \cite{1996_DraineBertoldi}, (3) \cite{1996_Lee}, (4) \cite{1997_NelsonLanger}}
\\
\endlastfoot
 k1 & \ce{H + e -> H+ + 2e}   &  ${\rm exp}[-32.71396786 $      & 1 \\
        &                                               & $ +13.536556 ~ \ln \TeV$                      & \\
        &                                               & $ -5.73932875 ~ (\ln \TeV )^2 $               & \\
        &                                               & $+1.56315498 ~ (\ln \TeV)^3$                  & \\
        &                                               & $-0.2877056 ~ (\ln \TeV)^4$                   & \\
        &                                               & $+3.48255977 \times 10^{-2} ~ (\ln \TeV)^5$   & \\ 
        &                                               & $-2.63197617 \times 10^{-3} ~ ( \ln \TeV)^6$  & \\
        &                                               & $+1.11954395 \times 10^{-4} ~ (\ln \TeV)^7$   & \\
        &                                               & $-2.03914985 \times 10^{-6} ~ (\ln \TeV )^8]$ & \\ 
k2      & \ce{H+ + e -> H + }$\gamma$   & $\exp[-28.6130338$                                                    & 1\\
                &                                               & $-0.72411256 ~ \ln \TeV $                                             & \\
                &                                               & $-2.02604473\e{-2}~ (\ln \TeV)^2$                             & \\
                &                                               & $-2.38086188\e{-3} ~ (\ln \TeV)^3$                            & \\
                &                                               & $-3.21260521\e{-4} ~ (\ln \TeV)^4$                            & \\
                &                                               & $-1.42150291\e{-5} ~ (\ln \TeV)^5$                            & \\
                &                                               & $+4.98910892\e{-6} ~ (\ln \TeV)^6$                            & \\
                &                                               & $+5.75561414\e{-7} ~ (\ln \TeV)^7$                            & \\
                &                                               & $-1.85676704\e{-8} ~ (\ln \TeV)^8$                            & \\
                &                                               & $-3.07113524\e{-9} ~ (\ln \TeV)^9]$                           & \\
        k12     & \ce{H2 + e -> 2H + e }                & $4.4\e{-10}~T^{0.35}\exp(-1.02\e{5}/T)$                               & 1\\ 
        k13     & \ce{H2 + H -> 3H}                             & $k_{\rm H}(k_{\rm L}/k_{\rm H})^a$,                                                   & 1\\
                &                                               &$k_{\rm L}\equiv 1.12\e{-10}\exp(-7.035\e{4}/T)$,                      &\\
                &                                               & $k_{\rm H}\equiv 6.5\e{-7}/\sqrt{T} ~ \exp(-5.2\e{4}/T)(1-\exp(-6000/T))$             & \\
                &                                               & $\log n_{\rm cr}\equiv{4-0.416\log(T/1.0\e{4})-0.327(\log(T/1.0\e{4}))^2}$,& \\
                &                                               & $a\equiv(1 +\nh/n_{\rm cr})^{-1}$                                     & \\
        k19     & \ce{3H -> H2 + H}                     & $5.5\e{-29}/T$                                                                & 1\\
        k20     & \ce{2H + H2 -> 2H2}           &$R_{\rm k19}/8$                                                                &1\\
        k21     &\ce{2H2 -> 2H + H2}            &$k_{\rm H}(k_{\rm L}/k_{\rm H})^a$,                                                            &1 \\
                &                                               &$k_{\rm L}\equiv1.18\e{-10}\exp(-6.95\e{4}/T)$,                        &\\
                &                                               &$k_{\rm H}\equiv8.125\e{-8}/\sqrt{T}\exp(-5.2\e{4}/T)(1-\exp(-6000/T))$,       & \\
                &                                               &$\log n_{\rm cr}\equiv{4.845-1.3\log(T/1.0\e{4})+1.62(\log(T/1.0\e{4}))^2}$,&\\
                &                                               &$a\equiv(1+\nh/n_{\rm cr})^{-1}$                                               &\\
        k22     &\ce{2H -> H+ + e + H}          &$1.7\e{-4}~R_{\rm k1}$                                                         & 1\\
        k23     &\ce{2H  ->C[dust] H2}          &$6.0\e{-17}\sqrt{T/300}~f_a~(\metal/\smetal)$                                          & 1\\
                &                                               &$ \times [1.0+4.0\e{-2}\sqrt{T+T_{\rm dust}}+2.0\e{-3}T+8.0\e{-6}T^2]^{-1}$,&\\
                &                                               &$f_a\equiv[1.0+\exp(7.5\e{2}(1/75-T_{\rm dust}^{-1}))]^{-1}$   & \\ 
        p1      &\ce{H} + $\gamma$ \ce{-> H+ + e}& $R_{\rm Ionize}$ ~(cf. \eqnref{eq:ioni})                                                     & -     \\
        p2      &\ce{H2} + $\gamma$ \ce{-> 2 H} & $R_{\ce{H2},\rm diss}$ ~(cf. \appref{sec:h2diss})                                                                                     & 2     \\
        p3      &\ce{CO} + $\gamma$ \ce{-> C+ + O}      &$R_{\ce{CO}, \rm diss}$        ~(cf. \appref{sec:codiss})              & 3 \\  
        k24     &\ce{C+ + O -> CO}                      &       $R_{\rm CO, form}$      ~(cf. \appref{sec:c_chain})                     & 4 %\\
%\hline
%\end{tabular}
%\end{center}
\label{tab:chem_reac}
\end{longtable}
}

        
        The azimuthal component of the hydrodynamics equations 
        is discretized in an angular momentum conserving form. 
        This apparently distinguishes the divergence operator of the component 
        from those of other components, as \eqnref{eq:euler_phi}.
        Let $\bm{F}$ an arbitrary vector. The divergence operators are calculated as
        \gathering{
                \nabla \cdot \bm{F}
                        =       \frac{1}{r^2} \partialdif{}{r} r^2 \, F_r 
                        + \frac{1}{r \sin \theta} \partialdif{}{\theta} 
                        \sin \theta \, F_\theta         ,   \\
                \nabla ^l \cdot \bm{F}  
                        =       \frac{1}{r^3} \partialdif{}{r} r^3 \,F_r 
                        + \frac{1}{r \sin ^2 \theta} \partialdif{}{\theta}      
                        \sin ^2 \theta \, F_\theta      .
        }       
        The angular momentum transfer due to the viscous stress is not included. 
        The viscous timescale is much longer than the dynamical timescale 
        within which we solve the time evolution. 


        The governing equations are closed by giving the equation of state (EOS).
        We use the EOS for an ideal gas
        \gathering{
                e=\frac{kT}{\mu m_u(\gamma -1)}                                                 ,       \\
                P=  \frac{\rho k T}{\mu m_u}                                                            , \label{eq:eqofstate}
        }
        where $e$ is the specific energy of the gas, 
        $\gamma$ is the adiabatic index,  
        $k$ is the Boltzmann constant, 
        $T$ is the gas temperature, 
        $\mu$ is the mean molecular weight, 
        and $m_u$ is the atomic mass unit.
        The adiabatic index is given by
        \eq{
                \gamma = 1 + \frac{\abn{HI} + \abn{\HIImath} + \abn{\ce{H2}} + \abn{e}}
                {\dfrac{3}{2} \abn{HI} + \dfrac{3}{2} \abn{\HIImath} + \dfrac{5}{2}\abn{\ce{H2}} + \dfrac{3}{2} \abn{e}} .
                \label{eq:specific_heat}
        }
        The contribution from the heavy elements can be neglected in \eqnref{eq:specific_heat}
        because of their negligible abundances.
        The EOS provides the explicit form of $E $ and $H$
        \gathering{
                E =\frac{1}{2} \rho \bm{v} ^2  + \rho e = \frac{1}{2} \rho \bm{v} ^2  + \frac{P}{\gamma-1}      , 
                        \\
                H= E + P =       \frac{1}{2} \rho \bm{v} ^2  + \frac{\gamma P}{\gamma-1}                .       
        }
        
\fi

